A Schnyder-type drawing algorithm for 5-connected triangulations

We define some Schnyder-type combinatorial structures on a class of planar triangulations of the pentagon which are closely related to 5-connected triangulations. The combinatorial structures have three incarnations defined in terms of orientations, corner-labelings, and woods respectively. The wood incarnation consists in 5 spanning trees crossing each other in an orderly fashion. Similarly as for Schnyder woods on triangulations, it induces, for each vertex, a partition of the inner triangles into face-connected regions (5~regions here). We show that the induced barycentric vertex-placement, where each vertex is at the barycenter of the 5 outer vertices with weights given by the number of faces in each region, yields a planar straight-line drawing.

==> defs_llncs.tex <==
\usepackage{amssymb,amsmath}
\usepackage{stmaryrd,paralist}
\usepackage{bbm}
\usepackage{graphics,graphicx}

\usepackage[latin1]{inputenc}
\usepackage{subfigure}
%\usepackage[margin=1.4 in]{geometry}
\usepackage{hyperref,color}
\usepackage[dvipsnames]{xcolor}
\graphicspath{{Figures/}} 
\graphicspath{{./Figures/}}

\usepackage{url}

\newcommand{\llncs}[1]{}
%\newcommand{\addllncs}[1]{\textcolor{purple}{#1}}
\newcommand{\addllncs}[1]{#1}

\newcommand{\OB}[1]{\textcolor{blue}{OB: #1}}
\newcommand{\ob}[1]{\textcolor{blue}{#1}}
\newcommand{\EF}[1]{\textcolor{ForestGreen}{EF: #1}}
\newcommand{\ef}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\SL}[1]{\textcolor{red}{SL:#1}}
%\renewcommand{\sl}[1]{\textcolor{red}{#1}}


\newtheorem{theo}{Theorem}
\numberwithin{theo}{section}
\newtheorem{thm}[theo]{Theorem}
%
\newtheorem{lem}[theo]{Lemma}
%
%\newtheorem{lemma}[theo]{Lemma}

\newtheorem{prop}[theo]{Proposition}
%
%\newtheorem{claim}[theo]{Claim}
%\newtheorem{fact}[theo]{Fact}

\newtheorem{Def}[theo]{Definition}
%
%\newtheorem{definition}[theo]{Definition}

\newtheorem{cor}[theo]{Corollary}
%
%\theoremstyle{remark}
%\newtheorem{remark}[theo]{Remark}


\newenvironment{Remark}{
\refstepcounter{theo}
\smallbreak\noindent%
\textbf{Remark~\thetheo.}}%
{\medbreak}

\newcommand{\ds}{\displaystyle}
\def\ni{\noindent}

\def\Nir{N_i^{\mathrm{right}}}
\def\Nil{N_i^{\mathrm{left}}}

\newcommand{\cacher}[1]{}

\def\ZZ{\mathbb{Z}}
\def\NN{\mathbb{N}}

\def\bz{\mathbb{Z}}
\def\bn{\mathbb{N}}
\def\br{\mathbb{R}}
\def\rp{\mathbb{R}^+}


\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cM{\mathcal{M}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cO{\mathcal{O}}
\def\cR{\mathcal{R}}
\def\cT{\mathcal{T}}
\def\cAL{\mathcal{AL}}
 
\def\cW{\mathcal{W}}
\def\cL{\mathcal{L}}

\def\cX{\mathcal{X}}


\def\bA{\mathbf{A}}
\def\bE{\mathbf{E}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bO{\mathbf{O}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bAL{\mathbf{AL}}
\def\bT{\mathbf{T}}

\def\bBA{\mathbf{BA}}
\def\bBL{\mathbf{BL}}
\def\bBM{\mathbf{BM}}
\def\bBW{\mathbf{BW}}


\def\ab{\alpha/\beta}


\def\hC{\hat{C}}

\def\Gb{G_\bullet}
\def\hGb{\widehat{G}_\bullet}
\def\bGb{\overline{G}_\bullet}
\def\tGb{\widetilde{G}_\bullet}

\def\cAb{\cA_\bullet}
\def\cBb{\cB_\bullet}
\def\bAb{\overline{\cA}_\bullet}
\def\hAb{\widehat{\cA}_\bullet}
\def\hom{\widehat \om}


%\def\hH{\widehat{H}}
\newcommand{\Id}{\textrm{Id}}



\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand{\om}{\omega}
\newcommand{\si}{\sigma}
\newcommand{\eps}{\epsilon}
\renewcommand{\th}{\theta}


\newcommand{\Om}{\Omega}
\newcommand{\Ga}{\Gamma}
\newcommand{\De}{\Delta}
\newcommand{\Th}{\Theta}





\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}

\newcommand{\bal}{\ov{\al}}
\newcommand{\bbe}{\ov{\be}}
\newcommand{\bga}{\ov{\ga}}
\newcommand{\bde}{\ov{\de}}
\newcommand{\bth}{\ov{\th}}
\newcommand{\bPhi}{\ov{\Phi}}
\newcommand{\bPsi}{\ov{\Psi}}
\newcommand{\bTh}{\ov{\Th}}
\newcommand{\bLa}{\ov{\Lambda}}
\newcommand{\beeta}{\ov{\eta}}



\def\Gcr{G^{\times}}
\def\jp{\mathrm{jump}}
\def\Sigmacw{J_{\mathrm{cw}}}
\def\Sigmaccw{J_{\mathrm{ccw}}}
\def\Ginf{G^{\infty}}



\newcommand{\fig}[3]{\begin{figure}[h!]\begin{center}\includegraphics[#1]{#2.pdf}\end{center}\caption{#3}\label{fig:#2}\end{figure}}

\def\vi{\overrightarrow{V}_{\!\!i}}
%\def\set5{\{1,\ldots,5\}}
\def\set5{[1:5]}
\def\omt{\omega_3}
\def\omf{\omega_5}
\def\bdelta{\boldsymbol{\delta}}
\def\ove{\overrightarrow}





\newcommand{\ee}{\textbf{e}}
\newcommand{\ff}{\textbf{f}}
\newcommand{\vv}{\textbf{v}}
\newcommand{\xx}{\textbf{x}}
\newcommand{\yy}{\textbf{y}}

\newcommand{\sups}[1]{\textsuperscript{#1}}

\newcommand{\cwjump}{\textrm{cw-jump}}
\newcommand{\ccwjump}{\textrm{ccw-jump}}

\newcommand{\indeg}{\textrm{indeg}}
\newcommand{\outdeg}{\textrm{outdeg}}
\newcommand{\toward}{\textrm{in}}
\newcommand{\inweight}{\textrm{inweight}}
\newcommand{\pseudol}{\textrm{enclength}}

\def\cw{clockwise}
\def\ccw{counterclockwise}


\def\oR{\overline{R}}



\newcommand{\Hd}{H^\diamond}
\newcommand{\Gd}{G^\diamond}


